Benchmarking Differential Privacy and Federated Learning for BERT Models

Natural Language Processing (NLP) techniques can be applied to help with the diagnosis of medical conditions such as depression, using a collection of a person's utterances. Depression is a serious medical illness that can have adverse effects on how one feels, thinks, and acts, which can lead to emotional and physical problems. Due to the sensitive nature of such data, privacy measures need to be taken for handling and training models with such data. In this work, we study the effects that the application of Differential Privacy (DP) has, in both a centralized and a Federated Learning (FL) setup, on training contextualized language models (BERT, ALBERT, RoBERTa and DistilBERT). We offer insights on how to privately train NLP models and what architectures and setups provide more desirable privacy utility trade-offs. We envisage this work to be used in future healthcare and mental health studies to keep medical history private. Therefore, we provide an open-source implementation of this work.

==> depression-table-full.tex <==
\begin{table*}[h]
  \centering
  \caption{Averaged Test Accuracies of DP and Baseline models on Depression}
  \begin{tabular}{|c|c|c|c|c|}
  \hline
   \textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
   \hline 
    0.5	&{53.20 $\pm$ 22.04} &{56.43 $\pm$ 24.13}	&{42.76 $\pm$ 24.29}	&{54.44 $\pm$ 22.48}\\ 
    \hline
    5	&{44.59 $\pm$ 23.26}	&{45.85 $\pm$ 15.23}	&{55.09 $\pm$ 22.76}	&{56.75 $\pm$ 12.42}\\ 
    \hline
    15	&{58.80 $\pm$ 19.09} &{39.76 $\pm$ 9.67} 	&{63.81 $\pm$ 10.86}	&{60.35 $\pm$ 11.58}\\ 
    \hline
    $\infty$ (No noise)	&{75.81}	&{84.01} &{74.47}	&{64.52}\\ 
    \hline
  \end{tabular}
  
  \label{dpdep}
\end{table*}





\begin{table*}[h]
\centering
  \caption{Averaged Test Accuracies of FL and DPFL models on Depression}
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
   \textbf{}	&\textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
   \hline 
    \multirow{4}{2em}{IID}	&0.5	&{57.24 $\pm$ 23.28}	&{39.02 $\pm$ 35.95}	&{20.23 $\pm$ 20.43} &{58.10 $\pm$15.30}\\ 
    & 5	&{70.92 $\pm$ 0.84}	&{39.13 $\pm$ 35.78}	&{54.43 $\pm$ 18.54}	&{45.49 $\pm$ 18.32}\\ 
    & 15 &{55.03 $\pm$ 9.77} &{57.13 $\pm$ 20.18} 	&{51.42 $\pm$ 27.79}	&{54.71 $\pm$ 15.68}\\
    & $\infty$ (No noise)	&{79.91 $\pm$ 1.87}	&{79.86 $\pm$ 2.98} &{69.73 $\pm$ 2.19 }	&{78.13 $\pm$ 0.76 }\\ 
    \hline
    \multirow{4}{2em}{Non IID}	&0.5	&{56.42 $\pm$ 24.13}	&{51.54 $\pm$ 21.57}	&{20.73 $\pm$ 13.67} &{56.05 $\pm$ 17.58}\\ 
    & 5	&{65.36 $\pm$ 3.54}	&{51.54 $\pm$ 17.61}	&{49.32 $\pm$ 16.88}	&{64.24 $\pm$ 7.26}\\ 
    & 15 &{42.91 $\pm$ 16.41} &{42.51 $\pm$ 17.69} 	&{54.24 $\pm$ 17.29 }	&{59.23 $\pm$ 13.10}\\
    & $\infty$ (No noise)	&{73.72 $\pm$ 2.32}	&{74.58 $\pm$ 1.65} &{69.25 $\pm$ 2.04}	&{74.25 $\pm$ 1.78}\\ 
    \hline
  \end{tabular}
  
  \label{fldep}
\end{table*}



\begin{table*}[t]
  \centering
  \caption{Averaged Test Accuracies of DP and Baseline models on Sexual Harassment}
  \begin{tabular}{|c|c|c|c|c|}
  \hline
   \textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
   \hline 
    0.5	&{47.89 $\pm$ 4.44} &{38.79 $\pm$ 15.38}	&{38.48 $\pm$ 25.96}	&{48.35 $\pm$ 5.45}\\ 
    \hline
    5	&{51.13 $\pm$ 4.90}	&{42.77 $\pm$ 2.90}	&{36.86 $\pm$ 12.38}	&{51.08 $\pm$ 4.90}\\ 
    \hline
    15	&{51.27 $\pm$ 4.80} &{48.45 $\pm$ 5.36} 	&{47.06 $\pm$ 2.96}	&{54.97 $\pm$ 0.57}\\
    \hline
    $\infty$ (No noise)	&{83.56}	&{81.14} &{73.65}	&{56.16}\\ 
    \hline
  \end{tabular}
  
  \label{dpharassment}
\end{table*}


\begin{table*}[h!]
\centering
  \caption{Averaged Test Accuracies of FL and DPFL models on Sexual Harassment}
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
  \textbf{}	&\textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
  \hline 
     \multirow{4}{2em}{Centralized}	
     &0.5	&{47.43 $\pm$ 2.94}	&{48.45 $\pm$ 4.38}	&{48.35 $\pm$ 4.45} &{45.26 $\pm$ 0.12}\\
    & 5	&{51.38 $\pm$ 4.22}	&{54.65 $\pm$ 0}	&{36.47$\pm$ 19.22}	&{46.46 $\pm$ 1.56}\\ 
    & 15	&{41.49 $\pm$ 12.44} &{48.45 $\pm$ 4.38} 	&{47.31 $\pm$ 3.65}	&{49.19 $\pm$ 2.50}\\ 
    & $\infty$ (No noise) &{54.85 $\pm$ 24.3}	&{76.28 $\pm$ 0.11} &{65.77 $\pm$ 0.85}	&{72.44 $\pm$ 1.74}\\ 
    \hline
    \multirow{4}{2em}{FL-IID}	
    &0.5	&{47.43 $\pm$ 2.94}	&{48.45 $\pm$ 4.38}	&{48.35 $\pm$ 4.45} &{45.26 $\pm$ 0.12}\\
    & 5	&{51.38 $\pm$ 4.22}	&{54.65 $\pm$ 0}	&{36.47$\pm$ 19.22}	&{46.46 $\pm$ 1.56}\\ 
    & 15	&{41.49 $\pm$ 12.44} &{48.45 $\pm$ 4.38} 	&{47.31 $\pm$ 3.65}	&{49.19 $\pm$ 2.50}\\ 
    & $\infty$ (No noise) &{54.85 $\pm$ 24.3}	&{76.28 $\pm$ 0.11} &{65.77 $\pm$ 0.85}	&{72.44 $\pm$ 1.74}\\ 
    \hline
    \multirow{4}{2em}{FL-Non IID}	
    &0.5  &{51.13 $\pm$ 3.98}	&{52.33 $\pm$ 1.63} &{15.67 $\pm$ 19.02}	&{47.15 $\pm$ 2.55}\\ 
    & 5	&{48.45 $\pm$ 4.18}	&{50.25 $\pm$ 3.46} &{33.43 $\pm$ 10.92}	&{51.41 $\pm$ 4.19}\\ 
    & 15	&{50.15 $\pm$ 3.91}	&{48.46 $\pm$ 4.37}  &{45.44 $\pm$ 2.73} &{48.95 $\pm$ 5.20}\\
    & $\infty$ (No noise)	&{63.52 $\pm$ 2.25}	&{73.55 $\pm$ 2.95} &{60.47 $\pm$ 2.04}	&{64.21 $\pm$ 8.15}\\ 
    \hline
  \end{tabular}
  
  \label{flharassment}
\end{table*}


==> related_work_long.tex <==
In this section, the latest research on differential privacy (DP) and federated learning (FL) applications implemented on Natural Language Processing (NLP) models  are reviewed briefly with the widespread use of NLP especially in the field of health, research and development studies aimed at protecting privacy have also started to take place in the literature.
Since machine learning algorithms are data-hungry, privacy concerns can restrict them from running the models through the sensitive data. This causes researchers to pay growing attention to data security against the threat of data leakage~\cite{zhangprivacy20, GONG2020484, securecollab20}. %At that point privacy-enhancing approaches gain importance to keep developing AI algorithms with trust. Recently, the studies on differential privacy and federated learning come forward in the literature review.
At that point privacy-enhancing approaches gain importance to keep developing Natural Language Processing algorithms with trust. Recently, the studies on differential privacy and federated learning come forward in the literature review.
Differential privacy~\cite{Dwork2011, Dwork06} which will be mentioned in the next section, uses random noise to provide that the publicly visible information doesn’t change much if one individual in the dataset is removed. On the other hand, deep learning  techniques are used to earn text representation via neural models by language application~\cite{Bengio03, Mikolov13, devlin-etal-2019-bert}. And mostly, the input text gives individual information about the author, such as demographic data. Some sentiment analysis results show that user attributes can be detected easily~\cite{Dirk15, Rosso2019}.There have been studies training differentially private deep models with the formal differential privacy approach in the literature \cite{Abadi_2016, mcmahan2018learning, Yu_2019}. ~\citeauthor{preotiuc-pietro-etal-2015-analysis} showed that demographic information about the text's author can be predicted through linguistic cues in the text. To tackle this kind of privacy concerns,~\citet{naacl-2021-textgen} and ~\citet{li-etal-2018-towards} propose training models using adversarial learning to improve the robustness and privacy of neural representation in natural language generation and classification  tasks, respectively.

However, since the popular data processing method is through the centralized way, It is open to leakages during collection and processing. Data are distributed over different organizations under the privacy threat. Because of this factor, federated learning has come forward as another privacy-enhancing approach~\cite{mcmahan2017communicationefficient, yang2019federated, kairouz2021advances}. 
%
%The notion of federated learning is proposed by Google researchers  \cite{konecny2016federated, konecny2017federated, McMahan2016FederatedLO}.
%
They aim to build machine learning models based on data sets that are distributed across multiple devices without data leakage.~\citeauthor{Sarma21} show that it is possible to train data  multi-institutionally without centralizing or sharing the underlying physical data through federated learning. There have been studies focusing on coping with the statistical challenges ~\cite{smith2018federated, Zhao18} and security concerns~\cite{Segal17, geyer2018differentially}. There also have been studies to customize federated learning~\cite{chen2019federated, smith2018federated}. Google proposed a horizontal federated learning solution for Android phone model updates~\cite{McMahan2016FederatedLO}.~\citeauthor{Segal17} introduce 
% \FM{when you want to name the authors, use citeauthor instead of cite, and always write in present tense. Also, when describing prior work and also your own work, use present tense and not past} 
a secure aggregation scheme to guard aggregated user updates under their federated learning framework.
The work done by~\citeauthor{singh2020benchmarking} also conducts similar benchmarking experiments on healthcare data however their work is focused on image data and vision tasks. 


==> results.tex <==
% \begin{table}[h]
%   \centering
%   \caption{DP and Baseline models on Depression}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
%   \hline 
%     0.5	&\text{59.29}	&\text{71.41}	&\text{71.41}	&\text{28.59}\\ 
%     \hline
%     5	&\text{29.89}	&\text{28.27}	&\text{71.41}	&\text{42.65}\\ 
%     \hline
%     15	&\text{68.17} &\text{28.59} 	&\text{25.85}	&\text{48.30}\\ 
%     \hline
%     Infinity	&\text{75.81}	&\text{84.01} &\text{74.47}	&\text{64.52}\\ 
%     \hline
%   \end{tabular}
  
%   \label{mlalgo}
% \end{table}

% \begin{table}[h]
%   \centering
%   \caption{DP and Baseline models on Sexual Harassment}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
%   \hline 
%     0.5	&\text{52.84}	&\text{52.57}	&\text{54.37}	&\text{54.65}\\ 
%     \hline
%     5	&\text{54.37}	&\text{43.35}	&\text{22.05}	&\text{45.49}\\ 
%     \hline
%     15	&\text{53.40} &\text{45.35} 	&\text{50.49}	&\text{54.65}\\ 
%     \hline
%     Infinity	&\text{83.54}	&\text{81.14} &\text{73.65}	&\text{56.16}\\ 
%     \hline
%   \end{tabular}
  
%   \label{mlalgo}
% \end{table}

% \begin{table}[h!]
%   \caption{FL and DPFL models on Depression}
%   \begin{tabular}{|c|c|c|c|c|c|}
%   \hline
%   \textbf{}	&\textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
%   \hline 
%     \multirow{4}{2em}{IID}	&0.5	&\text{69.95}	&\text{71.40}	&\text{49.43} &\text{71.40}\\ 
%     & 5	&\text{69.95}	&\text{71.40}	&\text{63.48}	&\text{71.40}\\ 
%     & 15 &\text{50.56} &\text{71.40} 	&\text{70.92}	&\text{63.97}\\
%     & Infinity	&\text{78.99}	&\text{82.87} &\text{71.72}	&\text{78.99}\\ 
%     \hline
%     \multirow{4}{2em}{Non IID}	&0.5  &\text{69.30}	&\text{71.40} &\text{28.59}	&\text{31.34}\\ 
%     & 5	&\text{69.46}	&\text{71.40} &\text{28.59}	&\text{54.28}\\ 
%     & 15	&\text{61.87}	&\text{48.46}  &\text{31.66}	&\text{40.87}\\
%     & Infinity	&\text{75.44}	&\text{73.18} &\text{71.56}	&\text{74.47}\\ 
%     \hline
%   \end{tabular}
  
%   \label{mlalgo}
% \end{table}

% \begin{table}[h!]
%   \caption{FL and DPFL models on Sexual Harassment}
%   \begin{tabular}{|c|c|c|c|c|c|}
%   \hline
%   \textbf{}	&\textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
%   \hline 
%     \multirow{4}{2em}{IID}	&0.5	&\text{45.07}	&\text{45.35}	&\text{45.35} &\text{52.14}\\ 
%     & 5	&\text{54.64}	&\text{45.35}	&\text{55.20}	&\text{45.21}\\ 
%     & 15	&\text{54.64} &\text{45.35} 	&\text{52.42}	&\text{47.85}\\ 
%     & Infinity	&\text{70.59}	&\text{76.14} &\text{65.88}	&\text{71.01}\\ 
%     \hline
%     \multirow{4}{2em}{Non IID}	&0.5  &\text{54.50}	&\text{54.64} &\text{54.09}	&\text{45.76}\\ 
%     & 5	&\text{57.28}	&\text{54.64} &\text{11.92}	&\text{54.09}\\ 
%     & 15	&\text{54.78}	&\text{45.35}  &\text{48.95} &\text{45.07}\\
%     & Infinity	&\text{61.71}	&\text{72.67} &\text{60.74}	&\text{55.61}\\ 
%     \hline
%   \end{tabular}
  
%   \label{mlalgo}
% \end{table}


% \begin{table}[h]
%   \centering
%   \caption{Standard Deviation of DP and Baseline models on Sexual Harassment}
%   \begin{tabular}{|c|c|c|c|c|}
%   \hline
%   \textbf{Epsilon}	&\textbf{BERT}	&\textbf{RoBERTa}	&\textbf{DistillBERT}	&\textbf{ALBERT}\\
%   \hline 
%     0.5	&\text{}	&\text{15.38}	&\text{25.96}	&\text{5.45}\\ 
%     \hline
%     5	&\text{4.90}	&\text{2.90}	&\text{12.38}	&\text{4.90}\\ 
%     \hline
%     15	&\text{4.80} &\text{5.36} 	&\text{2.96}	&\text{0.57}\\ 
%     \hline
%     Infinity	&\text{0}	&\text{0} &\text{0}	&\text{0}\\ 
%     \hline
%   \end{tabular}
  
%   \label{mlalgo}
% \end{table}

